Boolean Percolation on Doubling Graphs

We consider the discrete Boolean model of percolation on graphs satisfying a doubling metric condition. We study sufficient conditions on the distribution of the radii of balls placed at the points of a Bernoulli point process for the absence of percolation, provided that the retention parameter of the underlying point process is small enough. We exhibit three families of interesting graphs where the main result of this work holds. Finally, we give sufficient conditions for ergodicity of the discrete Boolean model of percolation.

==> comandos.tex <==
%%%%% COMANDOS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\RequirePackage{xspace,amsmath,amsthm,stmaryrd}
%%Cristian-Sebas
\newtheorem{teo}{Theorem}
\newtheorem{defi}[teo]{Definition}
\newtheorem{eje}[teo]{Ejemplo}
\newtheorem{lem}[teo]{Lemma}
\newtheorem{pro}[teo]{Proposition}
\newtheorem{coro}[teo]{Corollary}
\newtheorem{obs}[teo]{Observation}
\newtheorem{fact}[teo]{Fact}
\newtheorem{rem}[teo]{Remark}
\newtheorem{proo}[teo]{Proof}

\def\bteo{\begin{teo}}
\def\eteo{\end{teo}} 
 \def\bdefi{\begin{defi}}
\def\edefi{\end{defi}} 
\def\beje{\begin{eje}}
\def\eeje{\end{eje}} 
\def\blem{\begin{lem}}
\def\elem{\end{lem}} 
\def\bpro{\begin{pro}}
\def\epro{\end{pro}} 
\def\bproo{\begin{proo}}
\def\eproo{\end{proo}}
\def\bcoro{\begin{coro}}
\def\ecoro{\end{coro}}     
\def\bob{\begin{obs}}
\def\eob{\end{obs}}
\def\bfact{\begin{fact}}
\def\efact{\end{fact}}
\def\brem{\begin{rem}}
\def\erem{\end{rem}}

\def\bteo{\begin{teo}}
\def\eteo{\end{teo}} 
 \def\bdefi{\begin{defi}}
\def\edefi{\end{defi}} 
\def\beje{\begin{eje}}
\def\eeje{\end{eje}} 
\def\blem{\begin{lem}}
\def\elem{\end{lem}} 
\def\bpro{\begin{pro}}
\def\epro{\end{pro}} 
\def\bproo{\begin{proo}}
\def\eproo{\end{proo}}
\def\bcoro{\begin{coro}}
\def\ecoro{\end{coro}}     
\def\bob{\begin{obs}}
\def\eob{\end{obs}}
\def\bfact{\begin{fact}}
\def\efact{\end{fact}}
\def\brem{\begin{rem}}
\def\erem{\end{rem}}


\def\square{\ifmmode\sqr\else{$\sqr$}\fi}
\def\sqr{\vcenter{
         \hrule height.1mm
         \hbox{\vrule width.1mm height2.2mm\kern2.18mm\vrule width.1mm}
         \hrule height.1mm}} 

\def\reff#1{(\ref{#1})}

\def\proof{{\noindent\bf Proof. }}

\def\N{{\mathbb N}}
\def\Z{{\mathbb Z}}
\def\R{{\mathbb R}}
\def\bbR{{\mathbb R}}
\def\E{{\mathbf E}}
\def\P{{\mathbf P}}
\def\L{{\mathbb L}}

\def\cR{{\mathcal R}}
\def\cA{{\mathcal A}}
\def\cT{{\mathcal T}}
\def\cU{{\mathcal U}}
\def\cK{{\mathcal K}}
\def\cG{{\mathcal G}}
\def\cB{{\mathcal B}}
\def\a{{\alpha}}
\def\J{J}
\def\tG{{\tilde{g}}}
\def\Lc{{\Lambda^c}}
\def\Lg{{\Lambda}}
\def\cB{{\mathcal B}}
\def\cF{{\mathcal F}}
\def\cJ{{\mathcal J}}
\def\cS{{\mathcal S}}
\def\cP{{\mathcal P}}
\def\ic{{\{i\}^c}}
\def\be{{\mathbf e}}
\def\one{{\mathbf 1}}
\def\hX{{\hat X}}
\def\cE{{\mathcal E}}
\def\cX{{\mathcal X}}
\def\cC{{\mathcal C}}
\def\hR{{\hat R}}
\def\hcX{{\hat{\mathcal{X}}}}
\def\hcR{{\hat{\mathcal{R}}}}
\def\Hf{{H^{\Phi}}}
\def\Hi{{H^{\Phi}_i}}
\def\Hie{{H^{\Phi}_{i,\,\eta}}}
\def\Hiz{{H^{\Phi}_{i,\,\zeta}}}
\def\O{{\Omega}}
\def\D{{\Delta}}
\def\d{{\delta}}
\def\ep{{\epsilon}}
\def\o{{\omega}}
\def\e{{\eta}}
\def\z{{\zeta}}
\def\x{{\xi}}
\def\r{{\rho}}
\def\FA{{\Phi_A}}
\def\FL{{\Phi_{\Lambda}}}
\def\La{{\Lambda}}
\def\la{{\nu}}
%\decimalpoint
\newcommand{\norm}[1]{\ensuremath{\|#1\|}}
\newcommand{\origin}{\ensuremath{ o }}
\newcommand{\interior}[1]{\operatorname{int}(#1)}


%% Conjuntos
%\newcommand{\bbR}{\mathbb{R}}
\newcommand{\IR}{I\kern -0.37 em R}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\IH}{I\kern -0.37 em H}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\IL}{I\kern -0.37 em L}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbRP}{\mathbb{RP}}
\newcommand{\bbRH}{\mathbb{RH}}
\newcommand{\bbCP}{\mathbb{CP}}
\newcommand{\bbCH}{\mathbb{CH}}
\newcommand{\0}{\varnothing}
%\renewcommand{\2}[1]{\wp(#1)}
\newcommand{\difsim}{\!\vartriangle\!}
\newcommand{\disjunta}{\stackrel{\scriptscriptstyle{\circ}}{\cup}}
\newcommand{\compl}[1]{#1^{\mbox{\fontsize{6}{10}\selectfont C}}}
%% outra opç?o de complemento \newcommand{\compl}[1]{#1^{\mbox{\fontsize{6}{10}\selectfont $\complement$}}}

%% Operadores lógicos
\newcommand{\sse}{\Leftrightarrow}
\newcommand{\bor}[1]{\mathcal{B}(#1)}

%% Acentos e sinais genéricos, tamanho de fonte
\newcommand{\til}[1]{\widetilde{#1}}
\renewcommand{\bar}[1]{\overline{#1}}
\newcommand{\bola}[1]{\overset{\,\,\,\,\mbox{}_{\mbox{}_\circ}}#1}
\newcommand{\scr}[1]{\scriptscriptstyle{#1}}

%% Combinatória
\newcommand{\binomio}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)\,}

%% Funç?es trigonométricas
\DeclareMathOperator{\sen}{sen}
\DeclareMathOperator{\arcsen}{arcsen}
\DeclareMathOperator{\senh}{senh}
\DeclareMathOperator{\tg}{tg}
\DeclareMathOperator{\cotg}{cotg}
\DeclareMathOperator{\cossec}{cossec}
\DeclareMathOperator{\arccotg}{arccotg}
\DeclareMathOperator{\arcsec}{arcsec}
\DeclareMathOperator{\arccossec}{arccossec}

%% Funç?es, operadores, álgebra linear, grupos, cálculo
\DeclareMathOperator{\Dom}{Dom}
\DeclareMathOperator{\Img}{Im}
\DeclareMathOperator{\Grafico}{Graf}
\renewcommand{\ker}{\mathrm{ker}\,}
\renewcommand{\dim}{\mathrm{dim}\,}
\newcommand{\End}{\mathrm{End}\,}
\newcommand{\Aut}{\mathrm{Aut}\,}
\newcommand{\Iso}{\mathrm{Iso}\,}
\newcommand{\solucao}{\ensuremath{\mathop{Sol}\nolimits}}
%\newcommand{\solucao}{\mathcal{S}}
\newcommand{\cardinalidade}{\mathsf{\#}\,}
\def\Ga{{\Gamma}}
\def\ga{{\gamma}}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norma}[1]{\lVert#1\rVert}
\newcommand{\presc}[2]{\langle #1, #2 \rangle}
\newcommand{\vet}[1]{\overrightarrow{#1}}
\newcommand{\proj}[2]{\mathop{proj}_{\displaystyle #2} \,#1}

\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Hess}{Hess}
\DeclareMathOperator{\hess}{hess}
%\renewcommand{\div}{\mathrm{div}\,}

%% logicos
\newcommand{\es}{\wedge}
\newcommand{\ous}{\vee}
\newcommand{\naos}{\neg}
\newcommand{\Vs}{\mathrm{V}}
\newcommand{\Fs}{\mathrm{F}}
\newcommand{\el}{\ensuremath{\mathop{\mathit{e}}}\xspace}
\newcommand{\implical}{\ensuremath{\mathop{\mathit{implica}}}\xspace}
%\newcommand{\implical}{\textsl{\sffamily implica}}
\newcommand{\oul}{\ensuremath{\mathop{\mathit{ou}}}\xspace}
\newcommand{\naol}{\ensuremath{\mathop{\mathit{n\tilde{a}o}}}}
\newcommand{\Vl}{\textsl{\sffamily  verdadeiro}\xspace}
\newcommand{\Fl}{\textsl{\sffamily  falso}\xspace}
\newcommand{\Vla}{\textsl{\sffamily  verdadeira}\xspace}
\newcommand{\Fla}{\textsl{\sffamily  falsa}\xspace}
\newcommand{\Vlas}{\textsl{\sffamily  verdadeiras}\xspace}
\newcommand{\Flas}{\textsl{\sffamily  falsas}\xspace}
\newcommand{\Vls}{\textsl{\sffamily verdadeiros}\xspace}
\newcommand{\Fls}{\textsl{\sffamily falsos}\xspace}
\newcommand{\implica}{\Rightarrow}
\newcommand{\ssel}{\Leftrightarrow}
\newcommand{\tautologia}{\mathbf{t}}
\newcommand{\contradicao}{\mathbf{c}}
%\renewcommand{\labelitemi}{$\sqbullet$}
%\newcommand{\mint}[1]{\bigl[\kern -0.27 em | #1 |\kern -0.27 em \bigr]}
\newcommand{\mint}[1]{\llbracket #1 \rrbracket}
\newcommand{\talque}{\,\ensuremath{|}\, }

%limites
\newcommand{\eps}{\varepsilon}
\newcommand{\limite}{\lim\limits_{n \rightarrow \infty}}
\newcommand{\limiti}[1]{\lim\limits_{#1 \rightarrow \infty}}
\newcommand{\limitex}[1]{\lim\limits_{x \rightarrow #1}}
\newcommand{\limiteh}[1]{\lim\limits_{h \rightarrow #1}}
\newcommand{\limitet}[1]{\lim\limits_{t \rightarrow #1}}
\newcommand{\Area}{\mathrm{\acute{A}rea}}
\newcommand{\umsobre}[1]{\ensuremath{% fraç?es melhoradas
    \frac{\raisebox{-.1ex}{\ensuremath{1}}}%
         {\raisebox{.2ex}{\ensuremath{#1}}}}}  
\newcommand{\unosobre}[1]{\ensuremath{\mathchoice%
    {\umsobre{#1}}%        display math mode
    {\nicefrac{1}{#1}}%   in-line math mode
    {\nicefrac{1}{#1}}%   scriptstyle
    {\nicefrac{1}{#1}}}}% scriptscriptstyle  
    
\newcommand{\soma}[3]{\sum\limits_{#1=#2}^{#3}}
\newcommand{\produto}[3]{\prod\limits_{#1=#2}^{#3}}

\newcommand{\converge}{\rightarrow}


\newcommand{\compcent}[1]{\vcenter{\hbox{$#1\circ$}}}
\newcommand{\comp}{\mathbin{\mathchoice{\compcent\scriptstyle}{\compcent\scriptstyle}{\compcent\scriptscriptstyle}{\compcent\scriptscriptstyle}}}

%%%Algebra linear e matrizes
\newcommand{\determinante}[1]{\left\vert#1\right\vert}
\newcommand{\matriz}[1]{\left(#1\right)}
\DeclareMathOperator{\cof}{cof}
\DeclareMathOperator{\adj}{adj}

%%%%%%%%%Desenho de Intervalos

%inicio fim ponto 1 ponto2 ,tipoaberto ou fechado 
\newcommand\Interval[6]{
\newrgbcolor{ttttff}{0.2 0.2 1}
\psset{xunit=1.0cm,yunit=1.0cm,algebraic=true,dotstyle=o,dotsize=3pt
0,linewidth=0.8pt,arrowsize=3pt 2,arrowinset=0.25}
\begin{pspicture*}(#1,-0.6)(#2,0.56)
\psaxes[labelFontSize=\scriptstyle,xAxis=true,yAxis=false,Dx=1,Dy=1,
ticksize=-2pt 0,subticks=2]{-}(0,0)(-2.26,-0.6)(6.56,0.56)
\psline[linewidth=1.6pt,linecolor=ttttff](#3,0)(#4,0)
\psdots[,dotsize=4.5pt,dotstyle=#5,linecolor=blue](#3,0)
\psdots[,dotsize=4.5pt,dotstyle=#6,linecolor=blue](#4,0)
\end{pspicture*}
}
%\Interval{-3}{8}{2}{4}{*}{o}

%intervalo simples
\newcommand\Intervals[4]{%
  \begin{tikzpicture}[text height=1ex]%
    \draw[<-] (0,0) -- (1,0); 
    \draw[{#3-#4}] (1,0) node[label=below:{#1}] {} -- (2,0)
node[label=below:{#2}] {};
    \draw[->] (2,0) -- (3,0);
  \end{tikzpicture}
}

%\Intervals{-3}{8}{(}{)}

%%%%%%%%%%%%%%% Observações e afazer
\newcommand{\todopequeno}[2]{\todo[caption={#2},color=green!40]{#1}}
\newcommand{\todomedio}[2]{\todo[caption={#2},color=yellow!70]{#1}}
\newcommand{\todogrande}[2]{\todo[caption={#2},color=orange!90]{#1}}
\newcommand{\todoestrutural}[2]{\todo[caption={#2},color=red!40]{#1}}
\newcommand{\comentario}[2]{\todo[caption={#2},color=blue!40]{#1}}

%%%%dimensão de assouad
\newcommand{\asdim}{\operatorname{dim}_{A}\left(\Gamma\right)}
\newcommand{\pc}{p_c}

\newcommand{\V}[1]{\mathit{V(#1)}}
% \newcommand{\Ea}[1]{\mathit{E#1}}
\newcommand{\cc}{\mathcal{C}}
\newcommand{\medida}[1]{\operatorname{m}(#1)}



